dAJC: A 2.02mW 50Mbps Direct Analog to MJPEG Converter for Video Sensor Node using Low-Noise Switched Capacitor MAC-Quantizer with Auto-Calibration and Sparsity-Aware ADC

With the advancement in the field of the Internet of Things(IoT) and Internet of Bodies(IoB), video camera applications using Video Sensor Nodes(VSNs) have gained importance in the field of autonomous driving, health monitoring, robot control, and security camera applications. However, these applications typically involve high data rates due to the transmission of high-resolution video signals, resulting from high data volume generated from the analog-to-digital converters (ADCs). This significant data deluge poses processing and storage overheads, exacerbating the problem. To address this challenge, we propose a low-power solution aimed at reducing the power consumption in Video Sensor Nodes (VSNs) by shifting the computation from the digital domain to the inherently energy-efficient analog domain. Unlike standard architectures where computation and processing are typically performed in digital signal processing (DSP) blocks after the ADCs, our approach eliminates the need for such blocks. Instead, we leverage a switched capacitor-based computation unit in the analog domain, resulting in a reduction in power consumption. We achieve a $\sim4X$ reduction in power consumption compared to digital implementations. Furthermore, we employ a sparsity-aware ADC, which is enabled only for significant compressed samples that contribute to a small fraction ($\le5\%$) of the total captured analog samples, we achieve a $\sim20X$ lower ADC conversion energy without any considerable degradation, contributing to the overall energy savings in the system.

==> Author_Bios/Biography.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Author_Bios/photo_KGK.jpg}}]
{Gaurav Kumar K}
 (S`19) (Graduate Student Member, IEEE) received a bachelor’s degree in Electronics and Telecommunication Engineering from Jadavpur University, Kolkata, India, in 2017. He is currently pursuing a Ph.D. degree in electrical and computer engineering with Purdue University, West Lafayette, IN, USA, working with Prof. Shreyas Sen. 
 
Before joining Purdue, he worked as a Network Experience manager in the telecom industry at Bharti Airtel, India. He has interned with the Advanced R\&D Discovery Team, Texas Instruments (TI) Kilby Labs, USA, during the summer of 2021, where he worked on designing RX front end circuits  for high speed electrical links. His research interests include mixed-signal IC design for low power and high-speed sensors and wireline links.
 
 He has served as Primary and Secondary Reviewer for multiple reputed conferences, including IEEE International Conference on VLSI Design (VLSID) and IEEE Custom Integrated Circuit Conference (CICC).
\end{IEEEbiography}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Author_Bios/Author_BC.jpg}}]
{Baibhab Chatterjee}
 (S`17, M`22) (Graduate Student Member, IEEE) received the B.Tech. degree in electronics and communication engineering from the National Institute of Technology (NIT), Durgapur, India, in 2011, and the M.Tech. degree in electrical engineering from IIT Bombay, Mumbai, India, in 2015. He is currently pursuing the Ph.D. degree with the School of Electrical Engineering, Purdue University, West Lafayette, IN, USA. His industry experience includes two years as a Digital Design Engineer/a Senior Digital Design Engineer with Intel, Bengaluru, India, and one year as a Research and Development Engineer with Tejas Networks, Bengaluru. His research interests include low-power analog, RF, and mixed-signal circuit design for secure biomedical applications.
 
 Mr. Chatterjee received the University Gold Medal from NIT, Durgapur, India, in 2011, the Institute Silver Medal from IIT Bombay in 2015, the Andrews Fellowship at Purdue University during 2017-2019, the HOST 2018 Best Student Poster Award (3rd), the CICC 2019 Best Paper Award (overall), the RFIC/IMS 2020 3MT Award (audience choice) and the Bilsland Fellowship at Purdue University during 2021-2022.
\end{IEEEbiography}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Author_Bios/Author_SS.jpg}}]
{Shreyas Sen} (S`06-M`11-SM`17) (Senior Member, IEEE) received the
Ph.D. degree in ECE from Georgia Tech, Atlanta,
GA, USA, in 2011.

He has over five years of industry research experience in Intel Labs, Hillsboro, OR, USA, Qualcomm,
Austin, TX, USA, and Rambus, Los Altos, CA,
USA. He is currently an Elmore Associate Professor of ECE \& BME, Purdue University, West
Lafayette, IN, USA. Dr. Sen is the inventor of the
Electro-Quasistatic Human Body Communication
(EQS-HBC), or Body as a Wire Technology, for
which, he was a recipient of the MIT Technology Review top-ten Indian
Inventor Worldwide under 35 (MIT TR35 India) Award. His work has been
covered by 250+ news releases worldwide, invited appearance on TEDx
Indianapolis, Indian National Television CNBC TV18 Young Turks Program,
NPR subsidiary Lakeshore Public Radio, and the CyberWire podcast. He has
authored/coauthored three book chapters, over 175 journal and conference
papers, and has 15 patents granted/pending. He serves as the Director for
the Center for Internet of Bodies (C-IoB). His current research interests span
mixed-signal circuits/systems and electromagnetics for the Internet of Things
(IoT), biomedical, and security.

Dr. Sen is a recipient of the NSF CAREER Award in 2020, the AFOSR
Young Investigator Award in 2016, the NSF CISE CRII Award in 2017, the
Intel Outstanding Researcher Award in 2020, the Google Faculty Research
Award in 2017, the Purdue CoE Early Career Research Award in 2021,
the Intel Labs Quality Award in 2012 for industry-wide impact on USB-C
type, the Intel Ph.D. Fellowship in 2010, the IEEE Microwave Fellowship in
2008, the GSRC Margarida Jacome Best Research Award in 2007, and nine
best paper awards, including IEEE CICC in 2019, 2021, and in IEEE HOST
2017–2020, for four consecutive years. His work was chosen as one of the
top-ten papers in the hardware security field (TopPicks 2019). He serves/has
served as an Associate Editor for IEEE SOLID STATE CIRCUITS LETTERS
(SSC-L), \textit{Frontiers in Electronics}, \textit{IEEE Design \& Test}, an Executive Committee Member of the IEEE Central Indiana Section and a Technical Program
Committee Member of the ACM Design Automation Conference (DAC), the
IEEE Custom Integrated Circuit Conference (CICC), Design, Automation and
Test in Europe (DATE), the ACM/IEEE International Symposium on Low
Power Electronics and Design (ISLPED), the International Conference on
Computer-Aided Design (ICCAD), the International Test Conference (ITC),
VLSI Design, among others. 
\end{IEEEbiography}

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************

